Normalized Diversification

Generating diverse yet specific data is the goal of the generative adversarial network (GAN), but it suffers from the problem of mode collapse. We introduce the concept of normalized diversity which force the model to preserve the normalized pairwise distance between the sparse samples from a latent parametric distribution and their corresponding high-dimensional outputs. The normalized diversification aims to unfold the manifold of unknown topology and non-uniform distribution, which leads to safe interpolation between valid latent variables. By alternating the maximization over the pairwise distance and updating the total distance (normalizer), we encourage the model to actively explore in the high-dimensional output space. We demonstrate that by combining the normalized diversity loss and the adversarial loss, we generate diverse data without suffering from mode collapsing. Experimental results show that our method achieves consistent improvement on unsupervised image generation, conditional image generation and hand pose estimation over strong baselines.

==> alg/cross-domain.tex <==

\begin{algorithm}[tb]
	\caption{Computed $\ldiv$}
	\label{alg::ndiv_grad}
	\begin{algorithmic}[1]
		\While {not converged}
		\State Sample a minibatch of input data $\{x_i\}_{i=1}^m$ from $\mathcal{X}$.
		\State (For conditional models) Generate latent vectors $c_i$ based on $x_i$.
		%\State Sample a minibatch of latent vectors $\{z_{ij}\}_{j=1}^{n}$ for each $(x_i, c_i)$.
		%\State Generate outputs with:  $y_{ij}=\gt(c_i,z_{ij})$.
		\State (Optional) Update $F$ based on $\{x_i, y_{ij}\}$.% with %task-specific gradients. e.g. If $F$ is a discriminator, $\phi =\phi +\eta \partial_{\phi} \mathcal L(\theta,\phi)$.
		\State Optimize w.r.t the generator $\theta =\theta  -\eta\partial_{\theta} \mathcal L(\theta)$.% -\eta \mathbb E_p[\max(\ldiv(\theta, p),0)]$.
		% \State Optimize w.r.t the generator $\theta =\theta +\mathbb E_p[\max(\mathcal R(\theta, p),0)]$ 
		% \State Optimize w.r.t the generator $\theta =\theta -\eta
		% \partial_{\theta} \mathcal L(\theta,\phi)$
		\EndWhile
		%\EndFunction
	\end{algorithmic}
\end{algorithm}


==> alg/single-domain.tex <==

\begin{algorithm}[tb]
	\caption{Training pipeline of unsupervised setting.}
	\label{alg::pipeline_single}
	\begin{algorithmic}[1]
		%\Function{Iterative Pose Refine}{}
		\While {not converged}
		\State Sample a minibatch of latent vectors   $\{z_i\}_{i=1}^n$.
		\State Generate outputs with:  $y_i=\gt(z_i)$.
		\State (Optional.) Update $F$ based on $\{y_i\}_{i=1}^n$.% with task-specific gradients. e.g. If $F$ is a discriminator, $\phi =\phi +\eta \partial_{\phi} \mathcal L(\theta,\phi)$.
		\State Optimize the generator $\theta =\theta  -\eta\partial_{\theta} \mathcal L(\theta)$.%$-\eta \mathbb E_p[\max(\ldiv(\theta, p),0)]$.
		\EndWhile
		%\EndFunction
	\end{algorithmic}
\end{algorithm}


==> fig/demo.tex <==
\begin{figure}[tb]
	\centering
	\includegraphics[width=240pt]{img_src/demo.pdf}
	\vspace{-25pt}
	\caption{With the \textbf{\textit{normalized diversification}}, we learn to encode the target space with the predefined latent space $\mathbb{R}^n$, where each dimension follows $U(0,1)$. By maintaining valid interpolation, the model safely extrapolates based on the current structure. Also, normalizing the pairwise distance gets the outputs universally distributed in a self-adaptive manner. Instead of dense unbiased samples, our method only requires the gradient of a case-specific validity checking function.}
	% \caption{Visualization on learning self-adaptive diversification on the generalized setting, where only the unary checking feedback is given. Our method automatically parametrize the target space with the predefined latent space $\mathbb{R}^n$, where each dimension follows $U(0,1)$. Because unbiased groundtruth samples are intractable, all existing generative methods cannot address the severe problem of mode collapse in this sparse-sample setting. Via the normalized diversification, we not only discover the latent states but also learn a distance-preserving full parametrization.}
	\label{fig::demo}
	\vspace{-10pt}
\end{figure}


==> fig/maindemo.first-page.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\begin{center}
\vspace{-10pt}
\maketitle
\vspace{-10pt}
\input{fig/maindemo.tex}
\vspace{-10pt}
\captionof{figure}{NotImplementedError.}
\label{fig::maindemo}
\vspace{5pt}
\end{center}
}]


==> fig/text2image.tex <==
\begin{figure}[tb]
	\centering
	\includegraphics[width=240pt]{img_src/vis_text2image.jpg}
	\caption{Qualitative results on zero-shot text-to-image translation on Oxford-102 Flowers dataset \cite{nilsback2008automated}. Given the text, we get improvements on both quality and diversity.}
	\label{fig::text2image}
	\vspace{-10pt}
\end{figure}


==> tables/gan_original.tex <==
\begin{table}[tb]
	\centering
	\caption{FID \cite{NIPS2017_7240} Results for image generation on multiple datasets. We use DCGAN \cite{radford2015unsupervised} as our baseline. For `Ours-1' and `Ours-1024', the number denotes the dimension of the features encoded in Eq.(\ref{eq::emd_y}) after $g_Y$ (which is the discriminator). We train each combination for 50 epochs and each experiment is repeated 10 times. }
	\label{tab::gan} 
	\begin{tabular}{|c||c|c|c|}
		\hline
		& MNIST & CIFAR-10 & CIFAR-100 \\
		\hline
		DCGAN \cite{radford2015unsupervised} & 4.22 $\pm$ 0.41 & 45.4 $\pm$ 1.9 & 46.2 $\pm$ 0.9 \\
		\hline
		Ours-1 & 3.93 $\pm$ 0.37 & 44.9 $\pm$ 1.5 & 45.5 $\pm$ 1.6 \\
		\hline
		Ours-1024 & \textbf{3.88} $\pm$ 0.22 & \textbf{44.8} $\pm$ 1.4 & \textbf{44.5} $\pm$ 1.6\\
		\hline
	\end{tabular}
\end{table}	


==> tex/abs_bc1.tex <==


%Generative models are powerful tools for modeling images and can be used to synthesize photo-realistic ones. When applied to solve an ill-posed problem that fundamentally has multiple or infinite solutions, which we refer to as multimodal modeling, e.g. recovering a 3D hand pose from a 2D images of an occluded hand, the generative model needs to synthesize multiple solutions, each of which being plausible specifically to the surrounding environment. 

%Generating diverse outputs therefore becomes a necessary target for this problem, but some specific models, like a vanilla 
Generating diverse yet specific data is the goal of generative adversarial network (GAN), but it suffers from the problem of mode collapse, %In this paper, 
we introduced the concept of normalized diversity, which aims to ensure safe interpolation and active extrapolation.  Normalized diversification encourage that the normalized distance between paired outputs  % normalized distance of corresponding latent variables up to a scale. 
This encourages the outputs to actively extrapolate towards the outer important states, % On the other hand, with normalization we can get a relaxed upper bound over the normalized distance of paired outputs, 
and leads to manifold unfolding over generated outputs as well as safe interpolation between valid latent variables. %These two nice properties combine for a complete paradigm for learning a better parameterization of the output space with the relative pairwise distance preserved. 
Experimental results show that our method achieves consistent improvement on unsupervised image generation over strong baselines. When applied to conditional generative models for tasks such as image translation and hand pose estimation, our approach gets promising results over state-of-the-art methods on multi-modality modeling and feature learning.

% Conventional generative models such as VAE or GAN are known for suffering mode collapse or invalid mapping problems. Recent approaches tried to solve these problem mostly via incorporating the prior knowledge on the structure of target distribution. However, in the multi-modal setting, only very sparse (mostly only one) ground-truth samples are available for each conditional input, resulting in large sampling bias (intractable structural information) and even more severe mode collapse. In this paper, we consider a generalized setting for using generative models to learn representations that we do not have access to prior knowledge on the structure of target distribution, which poses two major challenges: 1) The outputs are easily stuck in a subspace. 2) High-order information for the target distribution are intractable. To address both issues, we propose \textbf{normalized diversification}, a clean yet incredibly effective regularization via the normalized pairwise distance. By training the generator in a min-max manner, our models can automatically discover and parameterize the whole target space to learn better features. Our method is well supported by a two-fold theoretical analysis from both geometry and functionality perspectives. Experimental results show that even under the conventional setting where there exist dense unbiased samples, our method still surprisingly achieves consistent improvement on addressing mode collapse. On multimodal problems such as conditional image generation and hand pose estimation, our proposed approach gets much promising results over state-of-the-art methods on multi-modality modeling and feature learning. 


==> tex/abs_bc2.tex <==


%Generative models are powerful tools for modeling images and can be used to synthesize photo-realistic ones. When applied to solve an ill-posed problem that fundamentally has multiple or infinite solutions, which we refer to as multimodal modeling, e.g. recovering a 3D hand pose from a 2D images of an occluded hand, the generative model needs to synthesize multiple solutions, each of which being plausible specifically to the surrounding environment. 

%Generating diverse outputs therefore becomes a necessary target for this problem, but some specific models, like a vanilla 
Generating diverse yet specific data is the goal of generative adversarial network (GAN), but it suffers from the problem of mode collapse. %In this paper, 
We introduced the concept of normalized diversity which forced the model to preserve the normalized pairwise distance between the sparse samples from a latent parametric distribution and their corresponding high-dimensional outputs. The normalized diversification aims to unfold the manifold of unknown topology and non-uniform distribution, which 
%enforces the efficient parameterization of the high-dimensional output by using the compact coding space and thus 
leads to safe interpolation between valid latent variables. By alternating the maximization over the pairwise distance and updating the total distance (normalizer), we encourage the model to actively explore in the high-dimensional output space. We demonstrate that by combining the normalized diversity loss and the adversarial loss, we generate diverse data without suffering from mode collapsing. 
%Through freezing the gradient in the  normalizer,  of the normalized pairwise distance, our model could
%perform efficient extrapolation in high-dimensional space b
%by leveraging the advantage of safe interpolation and more samples from the valid dataset, and the output geometric structure of current model. %This encourages the outputs to actively and effectively extrapolate towards the outer important states.
%We aim to expand and unfold manifold Normalized diversification encourage that the normalized distance between paired outputs  % normalized distance of corresponding latent variables up to a scale. 
 % On the other hand, with normalization we can get a relaxed upper bound over the normalized distance of paired outputs, 
%and leads to manifold unfolding over generated outputs as well as safe interpolation . 
%These two nice properties combine for a complete paradigm for learning a better parameterization of the output space with the relative pairwise distance preserved. 
Experimental results show that our method achieves consistent improvement on unsupervised image generation, conditional image generation and hand pose estimation over strong baselines. %Our approach gets promising results over state-of-the-art methods on multi-modality modeling and feature learning.

% Conventional generative models such as VAE or GAN are known for suffering mode collapse or invalid mapping problems. Recent approaches tried to solve these problem mostly via incorporating the prior knowledge on the structure of target distribution. However, in the multi-modal setting, only very sparse (mostly only one) ground-truth samples are available for each conditional input, resulting in large sampling bias (intractable structural information) and even more severe mode collapse. In this paper, we consider a generalized setting for using generative models to learn representations that we do not have access to prior knowledge on the structure of target distribution, which poses two major challenges: 1) The outputs are easily stuck in a subspace. 2) High-order information for the target distribution are intractable. To address both issues, we propose \textbf{normalized diversification}, a clean yet incredibly effective regularization via the normalized pairwise distance. By training the generator in a min-max manner, our models can automatically discover and parameterize the whole target space to learn better features. Our method is well supported by a two-fold theoretical analysis from both geometry and functionality perspectives. Experimental results show that even under the conventional setting where there exist dense unbiased samples, our method still surprisingly achieves consistent improvement on addressing mode collapse. On multimodal problems such as conditional image generation and hand pose estimation, our proposed approach gets much promising results over state-of-the-art methods on multi-modality modeling and feature learning. 


==> tex/intro_bc1.tex <==
% The concept of diversification is widely used in a variety of research fields including ecological science \cite{magurran1988diversity}, portfolio analysis \cite{solnik1974not}, recommendation system \cite{ziegler2005improving}, etc. The basic idea is to enable multiple reasonable choices for better stability and less bias towards the environment, the market and the user preference, etc. Recently, as the sampling bias has been the crucial challenge for representation learning, there has been increasing interest on data diversification such as offline augmentation and online hard negative mining. However, less effort has been put on promoting diverse valid outputs for learning better representations.
	
% Unsupervised representation learning from large-scale unlabeled datasets has continuously been a highly active topic in the past few years. The aim of the state-of-the art methods, such as VAE \cite{kingma2013auto} and GAN \cite{goodfellow2014generative}, are to attain better features via learning the target distribution from the dense unbiased samples in the datasets. The main challenge faced is the problem of mode collapse, which is when the model learns to generate only a few modes while many other modes are missed. Recently, this problem is addressed in much literature \cite{chen2016infogan, srivastava2017veegan, lin2017pacgan, xiao2018bourgan} by including either statistical or structural information of the target distribution.

%Problem: 

%Hand pose estimation
%Diversify
%{\jq introduction}
Diversity is an important concept in many areas, e.g. portfolio analysis \cite{solnik1974not}, ecological science \cite{magurran1988diversity} and recommendation system \cite{ziegler2005improving}. This concept is also crucial to generative models which have wide applications in machine learning and computer vision. %To begin with, we consider a simple example, the Gaussian Mixture Model (GMM), which is formed by multiple clusters. Each cluster of GMM has a different center and a covariance matrix, otherwise, GMM degenerates to Gaussian distribution and loses its advantage in modeling data with complex variations. The diversification of GMM is implicitly induced to the model when the objective function, i.e. log-likelihood, is maximized. More complex examples involve 
%Recently in deep learning, like  Variational Autoencoder (VAE) \cite{kingma2013auto} and the 
Several representative examples include the Variational Autoencoder (VAE) \cite{kingma2013auto}, Generative Adversarial Network (GAN) \cite{goodfellow2014generative}, which are capable of modeling complicated data.  One ideal principle shared by all generative models, simple or complex, is quite similar, that the generated data should be diversified. Otherwise, the model may have a so-called problem of mode collapse, where all generated outputs are highly similar. This problem is more common in GAN \cite{goodfellow2014generative} since the objective function is mostly about the validity of generated samples but not the diversity of them. 

The challenge for this problem is that we have to deal with very sparse samples, non-uniform distribution of the output data and unknown complex topology of target space.  We aim to learn a mapping to transform a latent variable in latent space $\mathcal Z$ to an image defined in output space $\mathcal Y$. However, we only have a very limited number of samples which are incapable of dealing with a much complicated topology of output data. This problem might be alleviated if the topology is simple since a parameterized function of smaller VC dimension might be able to fit, which, however, is most likely not the case if we need to deal with arbitrary images. %Plus, the non-uniform distribution of 

%{\jq interpolation and extrapolation} 
To learn a model that is meaningful and generalizable, we wish to achieve that the  \textit{interpolation} and \textit{extrapolation} on a pair of latent variables should generate valid samples in output space. This pursues a trade-off between pairwise diversity and validity.  This motivation aligns with the concept of \textit{local isometry} \cite{weinberger2006unsupervised},  which has a nice property that the near neighbors in $\mathcal Z$, are encoded to $\mathcal Y$ using a rotation plus a translation. Local isometry requires the image manifold to be smooth and without invalid `holes' within the neighbor region of a valid point, and the interpolation in $\mathcal Z$  generates valid points in $\mathcal Y$ through a parameterized mapping $\gt$ where $\theta$ is the parameter. Differently, Variational Autoencoder (VAE) \cite{kingma2013auto} mostly cares about local perturbation, or pointwise diversity. %Suppose $A, B$ are two generated points in a local region by the model, and a third point $C$ on a line through $A$ and $B$ by $C = \lambda A +(1-\lambda) B$ where $\lambda \in (0,1)$ results in an interpolation, and $\lambda \in (-\infty,0) \bigcup (1,+\infty)$ results in an extrapolation. Clearly, there is a slow transit from interpolation to extrapolation when $\lambda$ changes. 

%{\jq manifold unfolding}
In order to address the problem of mode collapse, we start from an idea that is orthogonal to previous research: that we aim to expand as well as unfold the manifold of generated images, actively and safely. %whereas [40] is only limited to matching a pre-defined manifold without exploration. 
As shown in Figure \ref{fig::donut-demo}, given a set of points, our goal is to discover the underlying parametrization so we can densely generate new valid samples in the interior (on the donut),  without crossing over to the exterior (the donut hole). To achieve this we utilize the same insight in manifold unfolding \cite{weinberger2006distance}. By pushing apart the pairwise distance of the sample points, we prevent the 'short-cuts' that links samples through the exterior space. In the donut case, given a triangulation on the samples, we try to expand the size of each triangle so that they don't fold over each other. Thus we can draw samples inside each triangle, which leads to better generalization. 

%	\begin{figure}[tb]
%		\centering
%		
%		\includegraphics[width=240pt]{concept.pdf}.pdf}
%	\vspace{-25pt}
%	\caption{ \textbf{\textit{normalized diversification}}, }
%	\vspace{-20pt}
%\end{figure}

% \noindent
% \textit{\textbf{1) Experimental illustration}}:  
%{\jq normalized diversity for inter and extro-polation}
In this paper, we propose \textit{normalized diversification} to encourage the learned mapping to preserve the normalized pairwise distance between every pair of inputs $z,z' \in \mathcal Z$ and their corresponding outputs $\gt(z),\gt(z') \in \mathcal Y $, where $\gt$ is a parameterized function. %This formulation has several nice properties on its own. 
We start with designing a regularization term that helps the generative model to maximize the pairwise distance  $\|\gt(z)-\gt(z')\|$, which also encourages the model to visit outer modes i.e. to extrapolate. Consequently, the objective function of the generative model based on extrapolated points helps to get the latent space extrapolation to be ``safe" as this operation generates valid samples. 
%second, by combining $\|z-z'\|$ and $\|\gt(z)-\gt(z')\|$, the model preserve the validity of interpolation in the input domain,
Suppose $A, B$ are two generated points in a local region by the model, and a third point $C$ on a line through $A$ and $B$ by $C = \lambda A +(1-\lambda) B$ where $\lambda \in (0,1)$ results in an interpolation, and $\lambda \in (-\infty,0) \bigcup (1,+\infty)$ results in an extrapolation. Clearly, there is a slow transition from interpolation to extrapolation when $\lambda$ changes.
%. The more interesting part is that this good property of interpolation will 
So the objective of safe extrapolation should, in turn, get the extrapolation in the next step ``safer" to more important outer states based on current structures. 
% Simply trying to enlarge the pairwise distance between samples explores unobserved space by extrapolation, but the crucial problem is how to make sure the interpolated point still to be valid. From a geometric perspective, imagine that $A, B, C$ are on a curvy $1D$ line in $2D$ space, the transitive distance from $d(A,B)$, $d(B,C)$ on the 1D curve is much longer than 2D distance $d(A,C)$, which violates the triangle inequality. If we make an interpolation point $D$ in the inner part of the line $(A,C)$, although the direct 2D distance between $d(A,C)$ could be very small, the line between them might lie in the part of unreasonable space out of the manifold. However, by pushing $(A,C)$ as far as possible away, we 'discover' the true 1D distance. 
% Another important property of this normalized diversification term is \textit{centralization}: that for each pair of samples $d(A,B)$, by normalizing the pairwise distance like ${d(A,B)}/{\mathbb E_C d(A,C)}$, each node is forced to be at the `center' of the embedding, and nobody is treated differently. Since if all the nodes are at the boundary of the embedding, the pairwise distances are large, but the normalization term scales equally so nothing changed. One way to achieve this goal of every sample being at the center, is to have circular or high-dimensional spherical embedding, where everyone is at the center. 

% {\jq centralization (optional, not decided using or not yet)}
% Another important property of using normalized pairwise distance is  \textit{centralization}: for each pair of samples $d(A,B)$, by normalizing the pairwise distance, each node is forced to be at the `center' of a valid node cluster. % the embedding. 
% The normalized pairwise distance on such embedding should diversify samples in each direction, plus, it will fix the scale ambiguity issue.
%If such encoding exists, we certainly could make an interpolation to be valid, since it is a linear relation. This property gets the encoding distributed universally. %One way to achieve this goal is to have circular or high-dimensional spherical embedding. 

Our paper is organized as follows: Section \ref{sec::motivation} presents more motivations towards a better understanding of diversification. Section \ref{sec::method} describes how we apply normalized diversification onto multiple vision applications by employing different metric spaces on the outputs. Finally in Section \ref{sec::exp}, we show promising experimental results on multiple tasks to demonstrate the effectiveness.
%The semi-definiteness of metric. 

% However, considering the multi-modal setting where the goal is to predict diverse valid outputs given a variable input, there are only very sparse (mostly only one) ground-truth samples available for each input. In these cases, simply applying deterministic models will result in a either biased or a mean (and maybe invalid) prediction. Moreover, either structural or statistical information is intractable, making the problem of mode collapse in the multi-modal setting even more severe. 

% In this paper, we consider a generalized setting for unsupervised representation learning. \textbf{Instead of dense unbiased samples, only the checking feedback is available. i.e. Direct sampling is extremely difficult.} The conventional setting can be viewed as a special case of this definition, where the checking feedback is whether the generated outputs are from the dense real samples. For the multi-modal setting, the problem can be included in the definition by designing task-aware checking feedback. This generalized setting poses two major challenges:

% \begin{itemize}
%  \item The outputs can easily stuck in a subspace, because we cannot attain sufficient knowledge towards the boundary and the statistics of the target distribution.
%  \item Both structural and statistical information for the target distribution are intractable, because we cannot have two or more unbiased ground-truth samples at a time.
% \end{itemize}

% To solve these hard issues, we propose a clean yet effective solution called normalized diversification. We employ the distance metric of both the latent space and the output space in a self-adaptive manner. Specifically, within a single batch, we get the normalized pairwise distance matrix of the outputs to be indexically lower bounded by that of the corresponding latent space samples. This regularization term is used in a min-max manner for optimizing the generator. Because the proposed method only utilizes unary feedback in the target space, it is able to be directly applied to all problems included in the generalized setting.

% Our method is theoretically grounded from both geometry and functionality perspectives. Results on a number of experiments are shown in Section \ref{sec::exp}. Even under conventional settings, without using high-order information in the dense unbiased samples, our method surprisingly gets promising results on addressing mode collapse. For multi-modal settings, which is the main focus of this work, our model achieves significant improvement on both quality and diversity on multiple tasks.

==> tex/method.1.tex <==
\label{sec::method}
In this section, we first define the generalized setting of learning representations via generative models, and then introduce the training pipeline  for applying {normalized diversification}. Finally, by employing different metric spaces $h_Y$ and checking {\jq (checking function needs to be defined, what is difference with objective or regularization function?)} function $F$, we show two examples on how our proposed normalized diversification can be integrated on multiple vision applications.

\subsection{Generalized Setting Formulation}
Implicit generative model based representation learning methods \cite{kingma2013auto,goodfellow2014generative} aim to fit data samples with a parametric distribution. We first go through the problem formulation for single-domain and cross-domain problems.

\begin{itemize}
	\item \textbf{Single-domain.} e.g. image synthesis, dialog generation. Existing methods such as GAN \cite{goodfellow2014generative} and VAE \cite{kingma2013auto} use a predefined latent space $\mathcal{Z}$  and learn the generative function $\gt:\mathcal{Z} \rightarrow \mathcal{Y}$ to fit the target $y \in \mathcal{Y}$ .
	\item \textbf{Cross-domain.} e.g. text-to-image (image-to-image) translation, pose estimation, future prediction. Related works include a variety of conditional generative models \cite{bao2017cvae, isola2017image, larsen2016autoencoding, reed2016generative, zhu2017toward}. Like single-domain cases, they also use a predefined latent space $\mathcal{Z}$ and aim to fit the joint distribution $(\mathcal{X}, \mathcal{Y})$ for the input domain $\mathcal{X}$ and output domain $\mathcal{Y}$ (for convenience we also use $\mathcal{Y}$ here). Specifically, an encoder $E:\mathcal{X}\rightarrow \mathcal{C}$ is used to get the latent code $c\in \mathcal{C}$. Then, either addition (VAE) or concatenation (CGAN) is employed to combine $c$ and $z$ and a generator $\gt:\mathcal{C}\times \mathcal{Z}\rightarrow \mathcal{Y}$ is trained.
\end{itemize}

Note that for both models, either $z\rightarrow y$ or $x\times z\rightarrow y$ {\jq  defining a  mapping should use space notation not variable} utilizes the gradient feedback by comparing the output $y$ with the dense ground-truth samples $\{y_r\}_{i=1}^n$. However, such dense samples are either expensive or intractable in many cases, especially in conditional cross-domain settings. For example, in multimodal tasks such as text-to-image translation and future prediction, given an input $x\in \mathcal{X}$, dense samples for $y|x$, $s.t.\quad y\in \mathcal{Y}$ are unavailable, resulting in intractable prior knowledge on either statistical or structural information of the conditional output $y|x$. 

Despite the stated difficulty, there does exist much information on the target space $y$ which can help estimate the validity or density on an output point $y_i$. For example, in the task of super resolution, there exist human priors that the down-sampled high-resolution images should be consistent with the low-resolution input. For pose estimation, the ambiguous occluded joints should be not only lying under the visible mask but also having some properties with respect to the object occluders. e.g. The hand pose should be like grabbing the cup if it is occluded by a held cup in the air. 
Thus, we consider a generalized setting where direct sampling on the target space is extremely difficult. Instead, only a checking module, $F(y) \text{ or } F(x,y)$, 
% \begin{equation}
%     F(y) \text{ or } F(x,y)
% \end{equation}
for single-domain (or cross-domain) setting is available. This means that only unary feedback can be utilized in an exploration manner. Note that for conventional single-domain settings, GAN \cite{goodfellow2014generative} lies in this generalized formulation for that $F$ can be interpreted as the trained discriminator. 

This generalized setting aims at how to transfer the prior knowledge $F$ to get better parameterization of the target space. $F$ can be not only the hand-crafted task-specific checking function based on human prior, but also be a discriminator either iteratively updated or pretrained and transferred from other tasks.

\subsection{Incorporating Normalized Diversification}
Motivated by the previously stated observations in Section \ref{sec::motivation}, we propose to use the \textbf{\textit{normalized diversification}} of the generator to learn a self-adaptive diversified parameterization. For every training step {\jq step or iteration? this term has to be consistent}, we force the outputs to not only extrapolate to visit more important states but also unwrinkle the inner structure to satisfy the interpolation property {\jq what is interpolation property? this sentence should be decomposed to make every word understandable} between the latent space and the outputs. 

%To be specific, given $N$ samples $\{z_i\}_{i=1}^N$ from the predefined latent space $\mathcal{Z}$ with prior distribution $p(z)$, we get the normalized distance matrix of the $N$ generated samples $\{\gt(z_i)\}_{i=1}^n$ to be indexically lower bounded by that of $\{z_i\}_{i=1}^n$.


%First, we use a soft constraint instead of the hard one in the objective function Eq.(\ref{obj1}), %. To put it formally, %we want the following equation to be a regularization term to the existing framework,
% %\begin{align}
% %\mathbb E_z [\|G(z) -G(z')\|^2 -\alpha \|z -z'\|^2] \geq 0,
% %\end{align}
% \begin{align}
% &\max_{\theta}\mathcal L(\theta,  p) +\mathbb E_p[\xi_{z,z'}],\\
% s.t.& \quad \mathcal R(\theta,z, z') + \xi_{z,z'} \geq 0, \quad \forall z,z',\quad \xi_{z,z'}\geq 0 \nonumber
% \end{align}
% where we take expectation to $z$ in the domain of interest. We should note that this objective function is a relaxation from another perspective, as we do not require the property to hold in every individual point. 
%  We approximate the expectation terms in Eq.(\ref{def:div_norm}) by
% \begin{align}\label{def:div_norm2}
% \dt(z,z')= \frac{N\|z -z'\|^2}{\sum_{i=1}^N \|z_i -z_i'\|^2}, %\dtt(z,z')=\frac{N\|z -z'\|^2}{\sum_{i=1}^N \|z_i -z_i'\|^2}.
% \end{align}
% Then we use a soft constraint instead of the hard one in the objective function, and the objective function can be written in a compact form as
% \begin{align*}
% \min_{\theta}\frac{1}{N}\sum_i^N\mathcal L(\theta,z_i) +\frac{1}{N^2}\sum_{i,j}^N [\max(\ldiv(\theta, z_i,z_j),0)].
% \end{align*}

The objective function has to be simplified to a form that only based on finite samples to implement, $\{z_i\}_{i=1}^N$ from $p(z)$. There exist two metric spaces $M_Z=(\mathcal{Z}, d_Z)$ and $M_Y=(\mathcal{Y}, d_Y)$. We use mapping functions $g_Z$ and $h_Y$ for embedding and then employ the Euclidean distance, as follows,
\begin{eqnarray}
%d_Z(z_i, z_j)=\|\phi_Z(z_i)-\phi_Z(z_j)\|_2
d_Z(z_i, z_j)=\|g_Z(z_i)-g_Z(z_j)\|_2
\label{eq::emd_z} \\
d_Y(y_i, y_j)=\|h_Y(y_i)-h_Y(y_j)\|_2
\label{eq::emd_y}
\end{eqnarray}
We define $D_Z, D_Y\in \mathbb{R}^{n\times n}$ to be the normalized pairwise distance matrix of $\{z_i\}_{i=1}^n$ and $\{y_i\}_{i=1}^n$ respectively in Eqs.(\ref{eq::ndistance_z} \ref{eq::ndistance_y}), where 
$D_Z=N_d(\{z_i\}_{i=1}^n, M_Z)$ and $D_Y=N_d(\{y_i\}_{i=1}^n, M_Y)$.
\begin{eqnarray}
(D_Z)_{ij} = (N_d(\{z_i\}_{i=1}^n, M_Z))_{ij}=\frac{d_Z(z_i, z_j)}{\sum_{\substack{j}} d_Z(z_i, z_j)}
\label{eq::ndistance_z} \\
(D_Y)_{ij} = (N_d(\{y_i\}_{i=1}^n, M_Y))_{ij}=\frac{d_Y(y_i, y_j)}{\sum_{\substack{j}} d_Y(y_i, y_j)}
\label{eq::ndistance_y}
\end{eqnarray}
Our divergence loss term on the generator can then be formulated as in Eq.(\ref{eq::div}), where $\alpha$ is the scaling factor of this regularization term.
\begin{equation}
\mathcal{L}_{div}= \|\max(\alpha D_Z-D_Y,0)\|_{L_1}
\label{eq::div}
\end{equation}

For each iteration at training stage, we constrain that the gradient is only backpropagated from the numerator. In this way, the generated samples $\{y_i\}_{i=1}^n$ in $\mathcal{Y}$ are forced to expand the space as well as implicitly regularize the structural behavior. This will put pressure on the weights of the generator $\gt$. The normalized version of the pairwise distance ensures that the property is scale-invariant. 

\subsection{Training Pipeline}
Our training pipeline is summarized in Algorithms \ref{alg::pipeline_single} and \ref{alg::pipeline_cross}. To get the outputs self-adaptive to the checking function $F(y)$ defined on $\mathcal{Y}$ (or $F(x,y)$ defined on $(\mathcal{X},\mathcal{Y})$), we include the normalized diversification $\mathcal{L}_{div}$ in Eq.(\ref{def:div}). The algorithm works in a push-and-pull manner. For each iteration, our system first update the checking function $F$ if $F$ is a discriminator, then we update $\gt$ with respect to the divergence term. Finally, we use the updated checking function to update $\gt$ again, putting pressure on invalid generated samples back to the target space. 

\input{alg/single-domain.tex}
\input{alg/cross-domain.tex}

\subsection{$h_Y$ as Nonlinear Embedding: Conditional Image Generation}
\label{sec::method_text2image}
In this section, we apply our proposed method onto the task of image generation. The simple single-domain image generation problem was initially addressed by VAE \cite{kingma2013auto} and GAN \cite{radford2015unsupervised}. Later, with the advent of CVAE and CGAN, cycle consistency and the help of human prior constraints, the application of cross-domain transfer including text-to-image \cite{reed2016generative}, image-to-image translation \cite{huang2018multimodal, Isola_2017_CVPR,zhu2017toward}, as well as super-resolution \cite{bulat2017super} was proposed. Considered as a multimodal {\jq multimodal has to be defined in the main text, as well as abstract} problem, cross-domain image transfer suffers much from the challenge of mode collapse and dataset overfitting. 

%Our method aims to simultaneously improve the quality and the diversity of the generated (single-domain) and translated images (cross-domain). 
To formulate the problem with the terminology used in previous sections, the output image domain is considered as $\mathcal{Y}$. However, defining a distance metric $d_Y$ on the high-dimensional image domain is a non-trivial problem. Recently, it was reported that \cite{zhangunreasonable} deep feature based perceptual metrics appear to be more consistent with human judgements than conventional metrics. Thus, we can use a pretrained embedding network as $h_Y$ to make the distance computationally affordable and semantically meaningful. Moreover, it is convenient to directly use the discriminators in GAN and CGAN formulation as the feature extractor $h_Y$. With $g_Z=I$ and the checking feedback $F$ being the discriminator itself, our proposed self-adaptive diversification can be integrated into GAN on image generation and CGAN on cross-domain transfer, following Algorithm \ref{alg::pipeline_single} and \ref{alg::pipeline_cross} respectively .

\subsection{$h_Y$ as Conditional Gating: Hand Pose Estimation}

Predicting 3D hand pose from RGB image is challenging due to heavy self occlusion and object occlusion from either egocentric or third-person viewpoint. When the hand is severely occluded, pose estimation in nature is a multi-modal problem. However, given a simple input RGB image, dense samples of conditional valid hand poses are obviously intractable. Normally, previous methods either leave the occluded joints unannotated \cite{mueller2017real} or label only one valid configuration over many possibilities. 

Actually, the pose estimation can be categorized into the cross-domain setting where $\mathcal{X}$ is the input image domain and $\mathcal{Y}$ is the 3D pose domain. However, the inherent ill-posed characteristics pose challenges onto the learning phase. On one hand, deterministic models will probably learn a conditional mean pose which is even not necessarily valid, resulting in relatively ineffective feature learning and inaccurate prediction. On the other hand, because there are limited samples of 3D poses for each input image, directly applying VAE \cite{kingma2013auto} or CGAN \cite{mirza2014conditional} will probably result in that the generator $\gt$ learns a many-to-one mapping from the latent space $\mathcal{Z}$ to 3D pose domain $\mathcal{Y}$. This will further degrade the generalization ability out of the training set.

By incorporating the self-adaptive diversification, we can get better parameterization towards the 3D pose space. In this case, we define $h_Y$ to be the gating function with respect to the occlusion mask. Specifically, we acquire the object masks and develop a pseudo-renderer by using morphological clues to get a coarse visibility mask $V\in \mathbb{I}^{21}$. We then use it to gate each joint of the output 3D pose for computing Eq.(\ref{eq::div}). i.e. $h_Y$ has the formulation below.

\begin{equation}
h_Y(y)=(1-V)\circ y
\end{equation}

In this way, we only put pressure {jq pressure?} on the occluded joints, making the ambiguity much clearer {alleviating the ambiguity}. For the checking function $F$ in our method, we choose to combine the hard $l_2$ distance on the visible joints and the joint adversarial discriminator of $(x_i, \hat{y}_i)$ (image-pose GAN), where $\hat{y}_i$ denotes the 2D projection of the output 3D pose $y_i$. 
\begin{align}
F(x,y)=F_{vis}(x,y)+F_{gan}(x,y)
\end{align} 
The two checking feedback {\jq the word feedback comes out suddenly, and this definition is introduced so late} are formulated below %in Eqs. \ref{eq::check_vis} and \ref{eq::check_gan}.
\begin{align}
&	F_{vis}(x, y)=\|V\circ (y-y_r)\|_2^2\\
\label{eq::check_vis}
F_{gan}(x, y)&=\mathbb{E}_{x,\hat{y}_r \sim p_{data}}[\log D(x, \hat{y}_r)] \\&+ \mathbb{E}_{x \sim p_{data}, z\sim p(z)}[\log(1- D(x, \hat{y}))]\nonumber
\label{eq::check_gan}
\end{align}
With the image-pose GAN, the system has the capability to learn much subtle relationship between $x$ and $y$. By constraining only on the visible joints, our system can learn better pose estimation along with better features in a weakly-supervised manner.


==> tex/method.temp.tex <==

% With the normalized diversification as soft constraints, we aim to guarantee that
% \begin{equation}
% \sum_{j=1}^n(NDy)_{ij}=1, \sum_{j=1}^n(NDz)_{ij}=1
% \label{eq::pr1}
% \end{equation}

% \begin{equation}
%     (NDy)_{ij}>\alpha (NDz)_{ij}
% \end{equation}

% For each $k \in \{1,2,...,n\}$,
% \begin{equation}
%     \sum_{j \neq k}^n(NDy)_{ij} > \alpha \sum_{j \neq k}^n(NDz)_{ij}
%     \label{eq::pr3}
% \end{equation}
% Because the normalization requires the sum of each row equals to 1 in Eq.(\ref{eq::pr1}), we can have the Eq.(\ref{eq::pr4}) from Eq. (\ref{eq::pr3}) as below:
% \begin{equation}
% 1-(NDy)_{ik} > \alpha(1-(NDz)_{ik})
% \label{eq::pr4}
% \end{equation}
% Thus, we have:
% \begin{equation}
% \alpha (NDz)_{ik} < (NDy)_{ik} < (1-\alpha) + \alpha (NDz)_{ik}
% \label{eq::pr5}
% \end{equation}
% Eq.(\ref{eq::pr5}) gives an relaxed upper bound for the normalized pairwise on the output $y$ space. This relaxed upper bound shall have similar properties with Lipschitz upper bound, which leads to manifold unfolding by maximizing the pairwise distance for the latent space $z$.

% Thus, the manifold unfolding comes from the normalization. 



==> tex/method_bc2.tex <==
\label{sec::method}
In this section, we present the real-world applicability of the proposed \textit{normalized diversification} and introduce the training pipeline for applying the term. By employing different metric spaces {built upon} $h_Y$ and an additional function $F$ to validate whether the image satisfy some task-specific constraints, to which we will refer as the checking function. For both kind of unsupervised and conditional models, %either $z\rightarrow y$ or $x\times z\rightarrow y$ {\jq  defining a  mapping should use space notation not variable} 
they utilize the gradient over the parameter by comparing the synthesized image $y$ with the samples from real-world $\{y_i\}_{i=1}^N$. However, a large amount of real images are either expensive or intractable in many cases, especially in conditional cross-domain settings. For example, in multimodal tasks such as text-to-image translation and future prediction, given an input $x\in \mathcal{X}$, dense samples for $y|x$, $s.t.\quad y\in \mathcal{Y}$ are unavailable, resulting in intractable prior knowledge on either statistical or structural information of the conditional output $y|x$. % We show two examples on how our proposed term can be integrated on multiple vision applications.

%\subsection{}
% Implicit generative model based representation learning methods \cite{kingma2013auto,goodfellow2014generative} aim to fit data samples with a parametric distribution. We first go through the problem formulation for single-domain and cross-domain problems.

% \begin{itemize}
% 	\item \textbf{Single-domain.} e.g. image synthesis, dialog generation. Existing methods such as GAN \cite{goodfellow2014generative} and VAE \cite{kingma2013auto} use a predefined latent space $\mathcal{Z}$  and learn the generative function $\gt:\mathcal{Z} \rightarrow \mathcal{Y}$ to fit the target $y \in \mathcal{Y}$ .
% 	\item \textbf{Cross-domain.} e.g. text-to-image (image-to-image) translation, pose estimation, future prediction. Related works include a variety of conditional generative models \cite{bao2017cvae, isola2017image, larsen2016autoencoding, reed2016generative, zhu2017toward}. Like single-domain cases, they also use a predefined latent space $\mathcal{Z}$ and aim to fit the joint distribution $(\mathcal{X}, \mathcal{Y})$ for the input domain $\mathcal{X}$ and output domain $\mathcal{Y}$ (for convenience we also use $\mathcal{Y}$ here). Specifically, an encoder $E:\mathcal{X}\rightarrow \mathcal{C}$ is used to get the latent code $c\in \mathcal{C}$. Then, either addition (VAE) or concatenation (CGAN) is employed to combine $c$ and $z$ and a generator $\gt:\mathcal{C}\times \mathcal{Z}\rightarrow \mathcal{Y}$ is trained.
% \end{itemize}


Despite the stated difficulty, there does exist much information on the target space $y$ which can help estimate the validity or density on an output point $y_i$. For example, in the task of super resolution, there exist human priors that the down-sampled high-resolution images should be consistent with the low-resolution input. For pose estimation, the ambiguous occluded joints should be not only lying under the visible mask but also having some properties with respect to the object occluders. e.g. The hand pose should be like grabbing the cup if it is occluded by a held cup in the air. 
Thus, we consider a generalized setting where direct sampling on the target space is extremely difficult. Instead, only a checking module, $F(y) \text{ or } F(x,y)$, 
% \begin{equation}
%     F(y) \text{ or } F(x,y)
% \end{equation}
for single-domain (or cross-domain) setting is available. This means that only unary feedback can be utilized in an exploration manner. Note that for conventional single-domain settings, GAN \cite{goodfellow2014generative} lies in this generalized formulation for that $F$ can be interpreted as the trained discriminator. This generalized setting aims at how to transfer the prior knowledge $F$ to get better parameterization of the target space. $F$ can be not only the hand-crafted task-specific checking function based on human prior, but also be a discriminator either iteratively updated or pretrained and transferred from other tasks.

% \subsection{Incorporating Normalized Diversification}
% Motivated by the previously stated observations in Section \ref{sec::motivation}, we propose to use the normalized diversification of the generator to learn a self-adaptive diversified parameterization. %For training {\jq step or iteration? this term has to be consistent}, 
% We force the outputs to not only extrapolate to visit more important states but also unwrinkle the inner structure to satisfy the interpolation property {\jq what is interpolation property? this sentence should be decomposed to make every word understandable} between the latent space and the outputs. 

%To be specific, given $N$ samples $\{z_i\}_{i=1}^N$ from the predefined latent space $\mathcal{Z}$ with prior distribution $p(z)$, we get the normalized distance matrix of the $N$ generated samples $\{\gt(z_i)\}_{i=1}^n$ to be indexically lower bounded by that of $\{z_i\}_{i=1}^n$.


%First, we use a soft constraint instead of the hard one in the objective function Eq.(\ref{obj1}), %. To put it formally, %we want the following equation to be a regularization term to the existing framework,
% %\begin{align}
% %\mathbb E_z [\|G(z) -G(z')\|^2 -\alpha \|z -z'\|^2] \geq 0,
% %\end{align}
% \begin{align}
% &\max_{\theta}\mathcal L(\theta,  p) +\mathbb E_p[\xi_{z,z'}],\\
% s.t.& \quad \mathcal R(\theta,z, z') + \xi_{z,z'} \geq 0, \quad \forall z,z',\quad \xi_{z,z'}\geq 0 \nonumber
% \end{align}
% where we take expectation to $z$ in the domain of interest. We should note that this objective function is a relaxation from another perspective, as we do not require the property to hold in every individual point. 
%  We approximate the expectation terms in Eq.(\ref{def:div_norm}) by
% \begin{align}\label{def:div_norm2}
% \dt(z,z')= \frac{N\|z -z'\|^2}{\sum_{i=1}^N \|z_i -z_i'\|^2}, %\dtt(z,z')=\frac{N\|z -z'\|^2}{\sum_{i=1}^N \|z_i -z_i'\|^2}.
% \end{align}
% Then we use a soft constraint instead of the hard one in the objective function, and the objective function can be written in a compact form as
% \begin{align*}
% \min_{\theta}\frac{1}{N}\sum_i^N\mathcal L(\theta,z_i) +\frac{1}{N^2}\sum_{i,j}^N [\max(\ldiv(\theta, z_i,z_j),0)].
% \end{align*}

% The objective function has to be simplified to a form that only based on finite samples to implement, $\{z_i\}_{i=1}^N$ from $p(z)$. There exist two metric spaces $M_Z=(\mathcal{Z}, d_Z)$ and $M_Y=(\mathcal{Y}, d_Y)$. We use mapping functions $g_Z$ and $h_Y$ for embedding and then employ the Euclidean distance, as follows,
% \begin{eqnarray}
% %d_Z(z_i, z_j)=\|\phi_Z(z_i)-\phi_Z(z_j)\|_2
% d_Z(z_i, z_j)=\|g_Z(z_i)-g_Z(z_j)\|_2
% \label{eq::emd_z} \\
% d_Y(y_i, y_j)=\|h_Y(y_i)-h_Y(y_j)\|_2
% \label{eq::emd_y}
% \end{eqnarray}
% We define $D_Z, D_Y\in \mathbb{R}^{n\times n}$ to be the normalized pairwise distance matrix of $\{z_i\}_{i=1}^n$ and $\{y_i\}_{i=1}^n$ respectively in Eqs.(\ref{eq::ndistance_z} \ref{eq::ndistance_y}), where 
% $D_Z=N_d(\{z_i\}_{i=1}^n, M_Z)$ and $D_Y=N_d(\{y_i\}_{i=1}^n, M_Y)$.
% \begin{eqnarray}
% (D_Z)_{ij} = (N_d(\{z_i\}_{i=1}^n, M_Z))_{ij}=\frac{d_Z(z_i, z_j)}{\sum_{\substack{j}} d_Z(z_i, z_j)}
% \label{eq::ndistance_z} \\
% (D_Y)_{ij} = (N_d(\{y_i\}_{i=1}^n, M_Y))_{ij}=\frac{d_Y(y_i, y_j)}{\sum_{\substack{j}} d_Y(y_i, y_j)}
% \label{eq::ndistance_y}
% \end{eqnarray}
% Our divergence loss term on the generator can then be formulated as in Eq.(\ref{eq::div}), where $\alpha$ is the scaling factor of this regularization term.
% \begin{equation}
% \mathcal{L}_{div}= \|\max(\alpha D_Z-D_Y,0)\|_{L_1}
% \label{eq::div}
% \end{equation}



\subsection{Training Pipeline}
Our training pipeline is summarized in Algorithms \ref{alg::pipeline_single} and \ref{alg::pipeline_cross}. To get the outputs self-adaptive to the checking function $F(y)$ defined on $\mathcal{Y}$ (or $F(x,y)$ defined on $(\mathcal{X},\mathcal{Y})$), we include the normalized diversification $\mathcal{L}_{div}$ in Eq.(\ref{eq::div}). The algorithm works in a push-and-pull manner. For each iteration, our system first update the checking function $F$ if $F$ is a discriminator, then we update $\gt$ with respect to the divergence term. Finally, we use the updated checking function to update $\gt$ again, putting pressure on invalid generated samples back to the target space. 

For each iteration at training stage, we constrain that the gradient is only backpropagated from the numerator. In this way, the generated samples $\{y_i\}_{i=1}^n$ in $\mathcal{Y}$ are forced to expand the space as well as implicitly regularize the structural behavior. This will put pressure on the weights of the generator $\gt$. The normalized version of the pairwise distance ensures that the property is scale-invariant. 
\input{alg/single-domain.tex}
\input{alg/cross-domain.tex}

\subsection{$h_Y$ as Nonlinear Embedding: Conditional Image Generation}
\label{sec::method_text2image}
In this section, we apply our proposed method onto the task of image generation. The simple single-domain image generation problem was initially addressed by VAE \cite{kingma2013auto} and GAN \cite{radford2015unsupervised}. Later, with the advent of CVAE and CGAN, cycle consistency and the help of human prior constraints, the application of cross-domain transfer including text-to-image \cite{reed2016generative}, image-to-image translation \cite{huang2018multimodal, Isola_2017_CVPR,zhu2017toward}, as well as super-resolution \cite{bulat2017super} was proposed. Considered as a multimodal problem, cross-domain image transfer suffers much from the challenge of mode collapse and dataset overfitting. 

%Our method aims to simultaneously improve the quality and the diversity of the generated (single-domain) and translated images (cross-domain). 
To formulate the problem with the terminology used in previous sections, the output image domain is considered as $\mathcal{Y}$. However, defining a distance metric $d_Y$ on the high-dimensional image domain is a non-trivial problem. Recently, it was reported that \cite{zhangunreasonable} deep feature based perceptual metrics appear to be more consistent with human judgements than conventional metrics. Thus, we can use a pretrained embedding network as $h_Y$ to make the distance computationally affordable and semantically meaningful. Moreover, it is convenient to directly use the discriminators in GAN and CGAN formulation as the feature extractor $h_Y$. With $g_Z=I$ and the checking feedback $F$ being the discriminator itself, our proposed self-adaptive diversification can be integrated into GAN on image generation and CGAN on cross-domain transfer, following Algorithm \ref{alg::pipeline_single} and \ref{alg::pipeline_cross} respectively .

\subsection{$h_Y$ as Conditional Gating: Hand Pose Estimation}

Predicting 3D hand pose from RGB image is challenging due to heavy self occlusion and object occlusion from either egocentric or third-person viewpoint. When the hand is severely occluded, pose estimation in nature is a multi-modal problem. However, given a simple input RGB image, dense samples of conditional valid hand poses are obviously intractable. Normally, previous methods either leave the occluded joints unannotated \cite{mueller2017real} or label only one valid configuration over many possibilities. 

Actually, the pose estimation can be categorized into the cross-domain setting where $\mathcal{X}$ is the input image domain and $\mathcal{Y}$ is the 3D pose domain. However, the inherent ill-posed characteristics pose challenges onto the learning phase. On one hand, deterministic models will probably learn a conditional mean pose which is even not necessarily valid, resulting in relatively ineffective feature learning and inaccurate prediction. On the other hand, because there are limited samples of 3D poses for each input image, directly applying VAE \cite{kingma2013auto} or CGAN \cite{mirza2014conditional} will probably result in that the generator $\gt$ learns a many-to-one mapping from the latent space $\mathcal{Z}$ to 3D pose domain $\mathcal{Y}$. This will further degrade the generalization ability out of the training set.

By incorporating the normalized diversification, we can get better parameterization towards the 3D pose space. In this case, we define $h_Y$ to be the gating function with respect to the occlusion mask. Specifically, we acquire the object masks and develop a pseudo-renderer by using morphological clues to get a coarse visibility mask $V\in \mathbb{I}^{21}$. We then use it to gate each joint of the output 3D pose for computing Eq.(\ref{eq::div}). i.e. $h_Y$ has the formulation below.

\begin{equation}
h_Y(y)=(1-V)\circ y
\end{equation}

In this way, we only put pressure {jq pressure?} on the occluded joints, making the ambiguity much clearer {alleviating the ambiguity}. For the checking function $F$ in our method, we choose to combine the hard $l_2$ distance on the visible joints and the joint adversarial discriminator of $(x_i, \hat{y}_i)$ (image-pose GAN), where $\hat{y}_i$ denotes the 2D projection of the output 3D pose $y_i$. 
\begin{align}
F(x,y)=F_{vis}(x,y)+F_{gan}(x,y)
\end{align} 
The two checking feedback {\jq the word feedback comes out suddenly, and this definition is introduced so late} are formulated below %in Eqs. \ref{eq::check_vis} and \ref{eq::check_gan}.
\begin{align}
&	F_{vis}(x, y)=\|V\circ (y-y_r)\|_2^2\\
\label{eq::check_vis}
F_{gan}(x, y)&=\mathbb{E}_{x,\hat{y}_r \sim p_{data}}[\log D(x, \hat{y}_r)] \\&+ \mathbb{E}_{x \sim p_{data}, z\sim p(z)}[\log(1- D(x, \hat{y}))]\nonumber
\label{eq::check_gan}
\end{align}
With the image-pose GAN, the system has the capability to learn much subtle relationship between $x$ and $y$. By constraining only on the visible joints, our system can learn better pose estimation along with better features in a weakly-supervised manner.


==> tex/method_bc3.tex <==
\label{sec::method}
In this section, we present the real-world applicability of normalized diversification with different metric spaces {built upon} $h_Y$. For both kinds of unsupervised and conditional models, %either $z\rightarrow y$ or $x\times z\rightarrow y$ {\jq  defining a  mapping should use space notation not variable} 
they utilize the gradient over the parameter by fitting the synthesized output $y$ with the samples from real-world $\{y_i\}_{i=1}^N$. %However, 
A large number of annotated images might be expensive to obtain. 
%in many cases, especially in conditional models as they need annotation. 
%For example, 
In conditional generation tasks such as text-to-image translation and future prediction, we need either dense samples of $y$ given input $x\in \mathcal{X}$, or additional constraints on the output space to which might lead to smaller statistical generalization error on the same function.  %resulting in intractable prior knowledge on either statistical or structural information of the conditional output $y|x$.
%Despite the stated difficulty, there does exist much information on the target space $y$ which can help estimate the validity or density on an output point $y_i$. 
For examples, in the task of super-resolution, %there %exist human priors that 
the down-sampled high-resolution images should be consistent with the low-resolution input. For pose estimation, the ambiguous occluded joints should be not only lying under the visible mask but also having some properties with respect to the object occluders, e.g. the hand pose should be like grabbing the cup if it is occluded by a held cup in the air. 
Thus, we consider a generalized setting where direct sampling on the target space is extremely difficult. We use an additional function $F$ to validate whether the generated sample satisfies some task-specific constraints, to which we will refer as the checking function. 
% Instead, only a checking module, $F(y) \text{ or } F(x,y)$, 
% % \begin{equation}
% %     F(y) \text{ or } F(x,y)
% % \end{equation}
% %for single-domain (or cross-domain) setting 
% is available. 
%This means that only unary feedback can be utilized for extrapolation. 
Note that for the unsupervised settings, GAN \cite{goodfellow2014generative} adopts a formulation that $F$ can be interpreted as the trained discriminator. Thus, we aim to transfer the prior knowledge from $F$ for a better parameterization of the target space. %$F$ can be not only the hand-crafted task-specific checking function based on human prior, but also be a discriminator either iteratively updated or pretrained and transferred from other tasks.

\subsection{Training Pipeline}
Our training pipeline is summarized in Algorithm \ref{alg::pipeline_cross}. To get the outputs satisfying the checking function $F(y)$ or $F(x,y)$, we include the term $\mathcal{L}_{div}$ in Eq.(\ref{eq::div}) for diversification. The algorithm %works in a push-and-pull manner. For each iteration, our system 
first updates the model parameter with respect to the checking function $F$, then updates $\gt$ with the diversity term and the checking function,  simultaneously putting penalties on invalid generated samples. 
%For each iteration at the training stage, we constrain that the gradient is only backpropagated from the numerator. This blocked gradient will encourage $\gt$ to extrapolate based on the current state. 
Within each iteration, we first calculate the denominator (the normalizer) of the normalized pairwise distance via forward propagation of the neural network, then use the gradient backpropagated from the numerator to update the model parameter, while fixing the denominator as a constant. This will greatly ease the calculation, and by our observation on massive experiments, has a side effect of stabilizing the training procedure to prevent the divergence of the objective function. We also conjecture that this modification possibly encourage $\gt$ to explore based on the current state based on our experiments. %In this way, the generated sample $y$ is forced to expand the space.% as well as implicitly regularize the structural behavior. 

% \subsection{$h_Y$ as Nonlinear Embedding: Conditional Image Generation}

\subsection{Conditional Image Generation}
\label{sec::method_text2image}
The normalized diversification can be used for the task of image generation. Pioneering works like VAE \cite{kingma2013auto} and GAN \cite{radford2015unsupervised} provided promising baselines for the unsupervised image generation problem. In later advance following these works, e.g. CVAE \cite{sohn2015learning} and CGAN \cite{mirza2014conditional}, great results were achieved on tasks like text-to-image synthesis \cite{reed2016generative}, image-to-image translation \cite{huang2018multimodal, Isola_2017_CVPR,zhu2017toward} and super-resolution \cite{bulat2017super}. %Considered as a multimodal problem, cross-domain image transfer suffers much from the challenge of 
However, most of those approaches tend to suffer from mode collapse or overfitting. 

%Our method aims to simultaneously improve the quality and the diversity of the generated (single-domain) and translated images (cross-domain). 
To formulate the problem with the terminology used in previous sections, the output image domain is considered as $\mathcal{Y}$. However, defining a distance metric $d_Y$ on the high-dimensional image domain is a non-trivial problem. Intuitively we can use $\ell_1$ or $\ell_2$ distance. Recently, it was reported that deep feature based perceptual metrics appear to be more consistent with human judgments than conventional metrics  \cite{zhangunreasonable}. Thus, it is convenient to directly use the discriminators in GAN and CGAN formulation as the feature extractor $h_Y$. With $h_Z(z)=z$ and the checking function $F$ being the discriminator like GAN, the diversification can be applied to unsupervised or conditional image generation, following Algorithm \ref{alg::pipeline_cross} respectively.

%\input{alg/single-domain.tex}
\input{alg/cross-domain.tex}
% \subsection{$h_Y$ as Conditional Gating: Hand Pose Estimation}
\subsection{Hand Pose Estimation}
\label{sec::posemethod}
Hand pose estimation is a crucial task towards understanding human activity and interaction. Predicting 3D hand pose from RGB image is challenging due to heavy self-occlusion and interactive occlusion from an unknown viewpoint, % When the hand is severely occluded, 
such pose estimation problem is intrinsically a ill-posed problem that requires a multimodel generator to synthesize. Given a simple input RGB image, enumerating unlimited number of 3D pose with the designated 2D pose that is also inaccurate, is considerably difficult.  Previous methods either leave the occluded joints with no annotation \cite{mueller2017real} or label only one valid configuration over many possibilities.  %Compared to the human body pose, the variations of hand poses are much subtle. Given an RGB image, the pose is likely to be ambiguous due to self-occlusion and object occlusion. 


Actually, the pose estimation can be categorized into the conditional generation setting where $\mathcal{X}$ is the input image domain and $\mathcal{Y}$ is the 3D pose domain. However, the inherent ill-posed characteristics pose challenges to the learning phase. On one hand, deterministic models will probably learn a conditional mean pose which is even not necessarily valid, resulting in relatively ineffective feature learning and inaccurate prediction. On the other hand, because there are limited samples of 3D poses for each input image, directly applying VAE \cite{kingma2013auto} or CGAN \cite{mirza2014conditional} will probably result in that the generator $\gt$ learns a many-to-one mapping from the latent space $\mathcal{Z}$ to 3D pose domain $\mathcal{Y}$. This will further degrade the generalization ability out of the training set.

By incorporating the normalized diversification, we can get a better parameterization of the 3D pose. In this case, we define $h_Y$ to be the gating function on the pose vector. We develop a pseudo-renderer by using morphological clues to get a mask $V\in \{0,1\}^{3K}$ to indicate the visibility of $K$ joints respectively. We use it to gate each joint of the output 3D pose for computing Eq.(\ref{eq::div}). i.e. $h_Y(y)=(1-V)\circ y$. %has the formulation below.
% \begin{equation}
% h_Y(y)=(1-V)\circ y
% \end{equation}
In this way, we only model the distance of poses on the visible joints, alleviating partial ambiguity from occlusion.  For the checking function $F$ in our method, we choose to combine the hard $l_2$ distance on the visible joints and the joint adversarial discriminator of $(x_i, \hat{y}_i)$ (image-pose GAN), where $\hat{y}_i$ denotes the 2D projection of the output 3D pose $y_i$. 
\begin{align}
F(x,y)=F_{vis}(x,y)+F_{gan}(x,y)
\end{align} 
The two checking functions %{\jq the word feedback comes out suddenly, and this definition is introduced so late} 
are formulated as follows %in Eqs. \ref{eq::check_vis} and \ref{eq::check_gan}.
\begin{align}
&	F_{vis}(x, y)=\|V\circ (y-y_r)\|_2^2\\
\label{eq::check_vis}
F_{gan}(x, y)&=\mathbb{E}_{x,\hat{y}_r \sim p_{data}}[\log D(x, \hat{y}_r)] \\&+ \mathbb{E}_{x \sim p_{data}, z\sim p(z)}[\log(1- D(x, \hat{y}))]\nonumber
\label{eq::check_gan}
\end{align}
With the image-pose GAN, the system has the capability to learn much subtle relationship between $x$ and $y$. By constraining only on the visible joints, our system gets less noisy gradients and can learn better pose estimation along with better image features.

\input{tables/5x5.tex}


==> tex/method_bc4.tex <==
\label{sec::method}
In this section, we present the real-world applicability of normalized diversification with different metric spaces {built upon} $h_Y$. For both kinds of unsupervised and conditional models, %either $z\rightarrow y$ or $x\times z\rightarrow y$ {\jq  defining a  mapping should use space notation not variable} 
they utilize the gradient over the parameter by fitting the synthesized output $y$ with the samples from real-world $\{y_i\}_{i=1}^N$. %However, 
A large number of annotated images might be expensive to obtain. 
%in many cases, especially in conditional models as they need annotation. 
%For example, 
In conditional generation tasks such as text-to-image translation and future prediction, we need either dense samples of $y$ given input $x\in \mathcal{X}$, or additional constraints on the output space to which might lead to smaller statistical generalization error on the same function.  %resulting in intractable prior knowledge on either statistical or structural information of the conditional output $y|x$.
%Despite the stated difficulty, there does exist much information on the target space $y$ which can help estimate the validity or density on an output point $y_i$. 
For examples, in the task of super-resolution, %there %exist human priors that 
the down-sampled high-resolution images should be consistent with the low-resolution input. For pose estimation, the ambiguous occluded joints should be not only lying under the visible mask but also having some properties with respect to the object occluders, e.g. the hand pose should be like grabbing the cup if it is occluded by a held cup in the air. 
Thus, we consider a generalized setting where direct sampling on the target space is extremely difficult. We use an additional function $F$ to validate whether the generated sample satisfies some task-specific constraints, to which we will refer as the checking function. 
% Instead, only a checking module, $F(y) \text{ or } F(x,y)$, 
% % \begin{equation}
% %     F(y) \text{ or } F(x,y)
% % \end{equation}
% %for single-domain (or cross-domain) setting 
% is available. 
%This means that only unary feedback can be utilized for extrapolation. 
Note that for the unsupervised settings, GAN \cite{goodfellow2014generative} adopts a formulation that $F$ can be interpreted as the trained discriminator. Thus, we aim to transfer the prior knowledge from $F$ for a better parameterization of the target space. %$F$ can be not only the hand-crafted task-specific checking function based on human prior, but also be a discriminator either iteratively updated or pretrained and transferred from other tasks.

%\subsection{Training Pipeline}
Our training pipeline is summarized in Algorithm \ref{alg::pipeline_cross}. To get the outputs satisfying the checking function $F(y)$ or $F(x,y)$, we include the term $\mathcal{L}_{div}$ in Eq.(\ref{eq::div}) for diversification. The algorithm %works in a push-and-pull manner. For each iteration, our system 
first updates the model parameter with respect to the checking function $F$, then updates $\gt$ with the diversity term and the checking function,  simultaneously putting penalties on invalid generated samples. 
%For each iteration at the training stage, we constrain that the gradient is only backpropagated from the numerator. This blocked gradient will encourage $\gt$ to extrapolate based on the current state. 

\input{alg/ndiv_grad.tex}
% \subsection{$h_Y$ as Nonlinear Embedding: Conditional Image Generation}
\subsection{Conditional Image Generation}
\label{sec::method_text2image}
The normalized diversification can be used for the task of image generation. Pioneering works like VAE \cite{kingma2013auto} and GAN \cite{radford2015unsupervised} provided promising baselines for the unsupervised image generation problem. In later advance following these works, e.g. CVAE \cite{sohn2015learning} and CGAN \cite{mirza2014conditional}, great results were achieved on tasks like text-to-image synthesis \cite{reed2016generative}, image-to-image translation \cite{huang2018multimodal, Isola_2017_CVPR,zhu2017toward} and super-resolution \cite{bulat2017super}. %Considered as a multimodal problem, cross-domain image transfer suffers much from the challenge of 
However, most of those approaches tend to suffer from mode collapse or overfitting. 

%Our method aims to simultaneously improve the quality and the diversity of the generated (single-domain) and translated images (cross-domain). 
To formulate the problem with the terminology used in previous sections, the output image domain is considered as $\mathcal{Y}$. However, defining a distance metric $d_Y$ on the high-dimensional image domain is a non-trivial problem. Intuitively we can use $\ell_1$ or $\ell_2$ distance. Recently, it was reported that deep feature based perceptual metrics appear to be more consistent with human judgments than conventional metrics  \cite{zhangunreasonable}. Thus, it is convenient to directly use the discriminators in GAN and CGAN formulation as the feature extractor $h_Y$. With $h_Z(z)=z$ and the checking function $F$ being the discriminator like GAN, the diversification can be applied to unsupervised or conditional image generation, following Algorithm \ref{alg::pipeline_cross} respectively.

% \subsection{$h_Y$ as Conditional Gating: Hand Pose Estimation}
\subsection{Hand Pose Estimation}
\label{sec::posemethod}
Hand pose estimation is a crucial task for understanding human activity and interaction.
Predicting 3D hand pose from RGB image is challenging due to self-occlusion.
%and interactive occlusion from an unknown viewpoint, % When the hand is severely occluded, 
This 3D pose estimation problem requires a multimodel generator to synthesize multiple 3D configurations all of which consistent with the 2D projection. Previous methods either leave the occluded joints with no annotation \cite{mueller2017real} or label only one valid configuration over many possibilities.  %Compared to the human body pose, the variations of hand poses are much subtle. Given an RGB image, the pose is likely to be ambiguous due to self-occlusion and object occlusion. 
Given a simple input RGB image, enumerating unlimited number of 3D pose with the designated 2D pose that is also inaccurate, is considerably difficult.

The pose estimation can be categorized into the conditional generation setting where $\mathcal{X}$ is the input image domain and $\mathcal{Y}$ is the 3D pose domain. However, the inherent ill-posed characteristics pose challenges to the learning phase. On one hand, deterministic models will probably learn a conditional mean pose which is even not necessarily valid, resulting in relatively ineffective feature learning and inaccurate prediction. On the other hand, because there are limited samples of 3D poses for each input image, directly applying VAE \cite{kingma2013auto} or CGAN \cite{mirza2014conditional} will probably result in that the generator $\gt$ learns a many-to-one mapping from the latent space $\mathcal{Z}$ to 3D pose domain $\mathcal{Y}$. This will further degrade the generalization ability out of the training set.

By incorporating the normalized diversification, we can get a better parameterization of the 3D pose. In this case, we define $h_Y$ to be the gating function on the pose vector. We develop a pseudo-renderer by using morphological clues to get a mask $V\in \{0,1\}^{3K}$ to indicate the visibility of $K$ joints respectively. We use it to gate each joint of the output 3D pose for computing Eq.(\ref{eq::div}). i.e. $h_Y(y)=(1-V)\circ y$. %has the formulation below.
% \begin{equation}
% h_Y(y)=(1-V)\circ y
% \end{equation}
In this way, we only model the distance of poses on the visible joints, alleviating partial ambiguity from occlusion.  For the checking function $F$ in our method, we choose to combine the hard $l_2$ distance on the visible joints and the joint adversarial discriminator of $(x_i, \hat{y}_i)$ (image-pose GAN), where $\hat{y}_i$ denotes the 2D projection of the output 3D pose $y_i$. 
\begin{align}
F(x,y)=F_{vis}(x,y)+F_{gan}(x,y)
\end{align} 
The two checking functions %{\jq the word feedback comes out suddenly, and this definition is introduced so late} 
are formulated as follows %in Eqs. \ref{eq::check_vis} and \ref{eq::check_gan}.
\begin{align}
&	F_{vis}(x, y)=\|V\circ (y-y_r)\|_2^2\\
\label{eq::check_vis}
F_{gan}(x, y)&=\mathbb{E}_{x,\hat{y}_r \sim p_{data}}[\log D(x, \hat{y}_r)] \\&+ \mathbb{E}_{x \sim p_{data}, z\sim p(z)}[\log(1- D(x, \hat{y}))]\nonumber
\label{eq::check_gan}
\end{align}
With the image-pose GAN, the system has the capability to learn much subtle relationship between $x$ and $y$. By constraining only on the visible joints, our system gets less noisy gradients and can learn better pose estimation along with better image features.

\input{tables/5x5.tex}


==> tex/motivation_bc1.tex <==
\label{sec::motivation}
% {\jq briefly talking about the problem}

We consider a generative model $\gt$ that generates an image $y \in \mathcal Y$ based on a latent variable $z$. The target of training the model is to fit an unknown target distribution $p(y)$ based on limited samples. In this paper, we consider two different kind of %problems via
implicit generative models that solving different problems but intrinsically share the same spirits of diversification. 
\begin{itemize}
	\item \textit{Unsupervised generative model.} This model is used for tasks that do not depend on auxiliary information, e.g. image synthesis without supervision. Existing methods such as GAN \cite{goodfellow2014generative} and VAE \cite{kingma2013auto} use a predefined latent space $\mathcal{Z}$  and learn the generative function $\gt:\mathcal{Z} \rightarrow \mathcal{Y}$ to fit the target $y \in \mathcal{Y}$.
	\item \textit{Conditional generative model. } This model utilizes additional information to generate more specific images, e.g. text-to-image (image-to-image) translation, pose estimation, future prediction. Related works include a variety of conditional generative models \cite{bao2017cvae, isola2017image, larsen2016autoencoding, reed2016generative, zhu2017toward}. Like single-domain cases, they also use a predefined latent space $\mathcal{Z}$ and aim to fit the joint distribution $(\mathcal{X}, \mathcal{Y})$ for the input domain $\mathcal{X}$ and output domain $\mathcal{Y}$ (for convenience we also use $\mathcal{Y}$ here). Specifically, an encoder $E:\mathcal{X}\rightarrow \mathcal{C}$ is used to get the latent code $c\in \mathcal{C}$. Then, either addition (VAE) or concatenation (CGAN) is employed to combine $c$ and $z$ and a generator $\gt:\mathcal{C}\times \mathcal{Z}\rightarrow \mathcal{Y}$ is trained.
\end{itemize}
The problem of mode collapse is frequently encountered especially in generative models like GAN \cite{goodfellow2014generative}, that the model generates highly similar data but satisfies the criterion for training. %This is in fact degenerated and meaningless. 
Our motivation for normalized diversification is to encourage $\gt$ to generate data with enough diversity, so the model visits most of the important modes. In the meantime, we wish  $\gt$ to be well-conditioned around the visited modes, so we could infer latent variables from some valid image samples, and ensure safe interpolation and extrapolation between these latent variables to generate meaningful images. %{\sh long and confused sentence which needs to be decomposed.} 
We could address the problem of mode collapse by diversifying the outputs, which is similar to enlarging the variance parameter of a Gaussian distribution, but a hard problem is how to measure the diversity of real-world images analytically and properly. For a Gaussian distribution, we may measure the diversity by its variance. But such formulation is neither universal nor adaptive. 

% {\jq defining normalized distance}
We start with an intuition to prevent the pairwise distance $d(\cdot,\cdot)$ between two generated points $A$ and $B$ from being too close. Note that if the outputs are linearly scaled, so will the pairwise distance $d(A,B)$: the samples seem to diversify from each other, without actually solving the intrinsic problem of mode collapse. 
%In the following context, we denote the model that we need to learn as $\gt(z)$ where $\theta$ is the parameter and $z \in \zsp$ is the input to the model. 
We measure whether the mapping preserves the normalized pairwise distance between inputs $\|z-z'\|$ and outputs $\|\gt(z)-\gt(z')\|$.

 %. %Actually, this problem is notorious for GAN and appears even more severe 
%especially in the multimodal case where only scarce samples is available.

% Without loss of generality, we assume to optimize the following objective function, $\mathcal L(\theta,  p)= \mathbb E_{p(z) }l(y,\gt(z))$ 
% % \begin{align}
% % \mathcal L(\theta,  p)= \mathbb E_{p(z) }l(y,\gt(z))
% % \end{align}
% where $y \in \mathcal Y$ denotes the target and $p$ characterizes the distribution of $z$, and $l$ is the loss function for individual pairs of inputs and outputs. 

% Particularly, we are interested in \textit{Lipchitz continuity} of the model: that $
% \gt(z)- \gt(z')  \leq L \|z-z'\|, \forall z,z' \in \mathbb R^{d}$,  % which are generally desired for basically most kinds of models. 
% %\begin{definition}
% % 	 $\gt$ satisfies% $L$-Lipchitz continuity if the following 
% % 	\begin{align}
% % 	\gt(z)- \gt(z')  \leq L \|z-z'\|, \forall z,z' \in \mathbb R^{d},
% % 	\end{align}
% where $L$ is a constant.
% %\end{definition} 
% %\begin{remark}
% In the sense that an ideal model changes only gradually w.r.t. to input variation, therefore could not incident an arbitrarily large variation in the output from a small noise on the input. %In statistical learning theory, the generation error of a neural network scales with the order of $\sqrt{L}$ with other conditions fixed, which indicates a tighter upper bound on the continuity gives a more generalized function to adapt to other data that are not available during training. 
% %\end{remark}


%During the training process, we certainly want to minimize a  regularized model with an adaptive loss term that reflects the diversity of the model output. 
Since we do not have access to infinite amount of data,  we sample a limited amount of data from a well-defined parametric distribution $p(z)$, and try to visit more mode via \textit{diversification}. We measure %by the distance of data pairs $\ldiv(\cdot,\cdot): \zsp \times \zsp \rightarrow \mathcal Y$ %that should maintain non-positive. 
% \begin{align}\label{obj1}
% \min_{\theta}\mathcal L(\theta,  p),\quad 
% s.t. \quad \ldiv(z, z') \leq 0, \forall z,z'
% \end{align}
%In our case, as we try to address the aforementioned mode collapse problem, we encourage the model to diverge so that it does not concentrated in one mode. 
%In a most naive way, we could measure the divergence of a model 
the diversity of generated samples by the pairwise distance in $\mathcal Y$ through the parameterized mapping $\gt$. The objective function has to be simplified to a finite-sum form on $N$ samples in latent space, $\{z_i\}_{i=1}^N$, along with corresponding images $\{y_i| y_i=\gt(z_i)\}_{i=1}^N$. We define two metric spaces $M_Z=(\mathcal{Z}, d_Z)$ and $M_Y=(\mathcal{Y}, d_Y)$. We use two additional functions $h_Y$ and $h_Z$ for some task-specific usage, and then define the metric as composite functions upon Euclidean distance, as follows,
\begin{align}
%d_Z(z_i, z_j)=\|\phi_Z(z_i)-\phi_Z(z_j)\|_2
d_Z(z_i, z_j)=\|h_Z(z_i) - h_Z(z_j)\|_2
\label{eq::emd_z} \\
d_Y(y_i, y_j)=\|h_Y(y_i)-h_Y(y_j)\|_2
\label{eq::emd_y}
\end{align}
%We briefly give an example about the definition and will give more details in the next section. 
To explain with a concrete application, here $d_Y$ may be used to measure the distance between hand poses under occlusion, with the prerequisite that $h_Y$ is defined to select visible landmarks of the hands, therefore only those joints are measured in the distance. 
% \begin{eqnarray}
% %d_Z(z_i, z_j)=\|\phi_Z(z_i)-\phi_Z(z_j)\|_2
% d_Z(z_i, z_j)=\|z_i-z_j\|_2
% \label{eq::emd_z} \\
% d_Y(y_i, y_j)=\|y_i-y_j\|_2.
% \label{eq::emd_y}
% \end{eqnarray}
We define $D^Z, D^Y\in \mathbb{R}^{N \times N}$ to be the normalized pairwise distance matrix of $\{z_i\}_{i=1}^N$ and $\{y_i\}_{i=1}^N$ respectively in Eqs.(\ref{eq::ndistance_z}). Each element in the matrix is defined as
%$D^Z=N_d(\{z_i\}_{i=1}^n, M_Z)$ and $D^Y=N_d(\{y_i\}_{i=1}^n, M_Y)$.
% \begin{eqnarray}
% (D^z)_{ij} = (N_d(\{z_i\}_{i=1}^n, M_Z))_{ij}=\frac{d_Z(z_i, z_j)}{\sum_{\substack{j}} d_Z(z_i, z_j)}
% \label{eq::ndistance_z} \\
% D^Y_{ij} = (N_d(\{y_i\}_{i=1}^n, M_Y))_{ij}=\frac{d_Y(y_i, y_j)}{\sum_{\substack{j}} d_Y(y_i, y_j)}
% \label{eq::ndistance_y}
% \end{eqnarray}
\begin{eqnarray}
D^Z_{ij} = \frac{d_Z(z_i, z_j)}{\sum_{\substack{j}} d_Z(z_i, z_j)}
\label{eq::ndistance_z}, \quad
D^Y_{ij}=\frac{d_Y(y_i, y_j)}{\sum_{\substack{j}} d_Y(y_i, y_j)}
\label{eq::ndistance_y},
\end{eqnarray}
for $\forall i, j \in[N]$. The diversity regularization on the generator can be formulated as in Eq.(\ref{eq::div}), where $\alpha >0$ is the scaling factor of this regularization term.
% \begin{equation}
% %\mathcal{L}_{div}= \|\max(\alpha D^z-D^Y,0)\|_{L_1}
% \mathcal{L}_{div}= \frac{1}{N^2} \sum_{i=1}^N \sum_{j=0}^N \max(\alpha D^z_{ij}-D^Y_{ij},0)
% \label{eq::div}
% \end{equation}
{%\sh
\begin{equation}
%\mathcal{L}_{div}= \|\max(\alpha D^z-D^Y,0)\|_{L_1}
\ldiv(\theta, h_Y, h_Z)= \frac{1}{N^2-N} \sum_{i=1}^N \sum_{j \neq i}^N \max(\alpha D^z_{ij}-D^Y_{ij},0)
\label{eq::div}
\end{equation}
}
A simple way of applying the divergence measure is to use it as a hard constraint, however, here we use it as a soft constraint, and the objective function can be written in a compact form as
\begin{align}
\min_{\theta} \mathcal L(\theta,p(z)) +\ldiv(\theta, h_Y, h_Z),
\end{align}
where $\mathcal L(\theta,p(z))$ is the original objective function for learning the generator $\gt$. In the conditional model, the objective function also depends on $x$ which we omitted here. % and the expectation is based on the latent variable distribution $p(z)$.
% We have a measurement of diversity
% \begin{align}\label{def:div}
% \ldiv(\theta, z,z')=\alpha \dtt(z, z')-  \dt(z, z'),
% \end{align}
% where $\alpha$ is a predefined hyper-parameter, and
% \begin{eqnarray}%\label{eq::emd_z}
% %d_Z(z_i, z_j)=\|\phi_Z(z_i)-\phi_Z(z_j)\|_2
% \dt(z, z')=\|\gt(z)-\gt(z')\|^2,\quad  % \\
% \dtt(z, z')=\|z-z'\|^2
% %\label{eq::emd_y}
% \end{eqnarray}
% this takes the intrinsic diversity of $z$ into account. This function measure whether the model preserves the pairwise distance sufficiently through the nonlinear transformation $\gt$. %Similar intuitions have been applied to subspace embedding methods. 
%By adding a variance term to to the objective function, the model is encouraged to visit a state in the image space that has is far away from the modes, as such states have lower probabilities of being visited if the covariance matrix has a smaller spectral norm.
%A function has $\tau$-gradient dominance property if it satisfies
%\begin{align}
%\gt(z)- \min_{z'}\gt(z')  \leq \frac{\tau}{2} \|\nabla \gt(z) \|^2, \forall z \in \mathbb  R^{d}.
%\end{align}
%An attractive property of this property is that the optimization algorithm finds a local minimum faster if the constant $\tau$ becomes tighter.  Taking the most common gradient descent algorithm for example, the running time for achieving an $\epsilon$-suboptimal solution scales with $\tau \log (1/\epsilon)$.
%\input{fig/donut_plot.tex}
\subsection{ Experimental illustration}
Figure \ref{fig::donut-demo} %\& \ref{fig::donut-curve} 
shows the results on recovering the data pattern (a donut) from sparsely sampled data. For quantitative evaluation, we discretized the donut region into uniform mesh grids and measured ``cover rate'' (the percentage of grids which have generated samples in them). This measure fits this case better than FID because it measures the real pattern instead of only comparing low-order moments of the samples. In addition, we measured ``outlier rate'': the ratio of samples outside the donut. It is shown that Ours fills in the holes and generates dense coverage while GAN and BourGAN fails to generalize. 

\subsection{Understanding from Geometric Perspective}
Simply trying to enlarge the pairwise distance between samples explores unobserved space by extrapolation, but a crucial problem is how to make sure the interpolated point still to be valid. From a geometric perspective, imagine that $A, B, C$ are on a curvy $1D$ line in $2D$ space, the transitive distance from $d(A,B)$, $d(B,C)$ on the 1D curve is much longer than 2D distance $d(A,C)$, which violates the triangle inequality. If we make an interpolation point $D$ in the inner part of the line $(A,C)$, although the direct 2D distance between $d(A,C)$ could be very small, the line between them might lie in the part of unreasonable space out of the manifold. However, by pushing $(A,C)$ as far as possible away, we 'discover' the true 1D distance. This insight is different from existing approaches, e.g. BourGAN \cite{xiao2018bourgan}, which aims at matching the pairwise distance between output space and latent space which can preserve the data modality but hinder its generalization ability. Our method, besides the mode preserving ability, can also actively expand and unfold the manifold. This benefits learning a robust encoding space without holes, which enables safe interpolation on the latent space where the generated samples will neither lie outside the valid region nor overfit the existing data (See Figure \ref{fig::donut-demo}).

An important motivation behind that we normalizing the diversity term is \textit{centralization}: that for each pair of samples $d(A,B)$, by normalizing the pairwise distance like ${d(A,B)}/{\mathbb E_C d(A,C)}$, each node is forced to be at the `center' of the embedding, and nobody is treated differently. Since if all the nodes are at the boundary of the embedding, the pairwise distances are large, but the normalization term scales equally so nothing changed. One way to achieve this goal of every sample being at the center, is to have circular or high-dimensional spherical embedding, where everyone is at the center. 

\input{fig/donut_demo.tex}
\subsection{Understanding via Linear Models}
%However, we must notice that this property alone does not prevent degenerated cases. 
To to understand the normalized diversification, we start from another perspective by using simple functions to illustrate the functionality of the regularization term. We assume the generator to a simple linear model as $\gt(z)=W^T z$, where % $\tilde \gt(z)$ is a nonlinear feature (e.g. produced by neural networks), and 
$W$ is the matrix that characterizes the linear transformation. A simple calculation induces that the diversity regularization thus encourages $\|W\|_{\star}$ (or $\|W\|_{2}$) being sufficiently large. However, this alone does not prevent some degenerated cases. Suppose that the generator is constructed in the following way %$\gt(z)= W^T \tilde \gt(z)_1$
\begin{align*}
\gt(z)= W^T z, W=diag[\beta ,0,0,\cdots,0] \in \mathbb R^{K \times K},
\end{align*}
%and the index $1$ represents the first element. W
where $K$ is the dimension of the latent variable $z$. When $\beta$ is sufficiently large, this generator seems to be strongly diversified, however, is actually not a reasonable model. Normalization over the diversity helps to prevent these kinds of degenerated cases, as the normalized distance does not scale with $\beta$. The normalization also helps to adapt to a conditional setting that some related works e.g. BourGAN \cite{xiao2018bourgan} might fail to adapt, based on an input variable $x$ and a latent variable $z$, especially with large variations w.r.t. $x$, such that  $||g(x,z)-g(x,z')||\leq \alpha ||z-z'||$. 
%if $g(\cdot,z)$ strongly changes w.r.t $y$, then the factor $\alpha$ in [40] has to be either too large to be meaningless to restrict $y$ (like a meaninglessly large Lipchitz constant to bound a function), or too small to cover all possible y. 
Imagine a simple example where $y=g(x,z) = (x+z)^3$, and $x \in [1,10]$. Then $\alpha \geq 3 {\max(x)}^2=300$. However, this $\alpha$ is meaningless for most parts of $[1,10]$. %This illustrates that [40] can not handle large variations in condition generation setting. 
Explicitly normalizing the divergence could fix $\alpha$ to a reasonable range.  
% we propose a normalized version of the diversity measure,
% \begin{align}\label{def:div_norm}
% %d_Z(z_i, z_j)=\|\phi_Z(z_i)-\phi_Z(z_j)\|_2
% \dt(z, z')&=\frac{\|\gt(z)-\gt(z')\|^2}{ \mathbb E_{p(z)}\|\gt(z)-\gt(z')\|^2},\nonumber\\% \\
% \dtt(z, z')&=\frac{\|z-z'\|^2}{ \mathbb E_{p(z)}\|z-z'\|^2}
% %\label{eq::emd_y}
% \end{align}

% \begin{align}\label{def:div_norm}
% \mathcal R(\theta, z,z')=\frac{\dt(z,z')}{ \mathbb E_{p(z)}\|\dt(z,z')\|^2}
% -\alpha \frac{\dtt(z,z')}{\mathbb E_{p} \dtt(z,z')}.
% \end{align}
%To understand this divergence measure from the geometric perspective, normalizing each pairwise distance $d(z,z')$ by the expectation of distance forces every node to be at the 'center' of the embedding (when it is close to everyone). This implies two points:
%1) we can not just push all the nodes to the boundary of the embedding, which is good for diversification, but not good for normalization term of $\mathbb E_{p(z)}\|\gt(z)-\gt(z')\|^2$; 2) one way to achieve this goal is to make circular or high-dimensional spherical embedding, where everyone is at the center. 

%To understand the divergence measure, we provide insights about how it works.  From a geometric perspective, imagine that $A, B, C$ are on a curvy $1D$ line in $2D$ space, the transitive distance from $d(A,B)$, $d(B,C)$ on the 1D curve is much longer than 2D distance $d(A,C)$, which violates the triangle inequality. If we make an interpolation point $D$ in the inner part of the line $(A,C)$, although the direct 2D distance between $d(A,C)$ could be very small, the line between them might lie in the part of unreasonable space out of the manifold. However, by pushing $(A,C)$ as far as possible away, we 'discover' the true 1D distance. From a function perspective, 

%We denote a simplified model as $\gt(z)=W^T \tilde \gt(z)$, where $\tilde \gt(z)$ is a nonlinear feature (e.g. produced by neural networks), and $W$ is the transformation matrix (the last layer). The constraint on the divergence function thus regularizes $\|W\|_{\star}$ (or $\|W\|_{2}$) being insufficiently large. 


% From the functionality perspective to understand, we seek to find a case that gives a strongly negative value of $\ldiv$. To start with, any $L$-Lipchitz function satisfies
% \begin{align}\label{def:bound1}
% \mathbb E \|\gt(z_i) -\gt(z_i')\|^2 \leq L^2 {\mathbb E\|z_i -z_i'\|^2}.
% \end{align}
% Note that this is actually a relaxed bound on the continuity. In addition, if the following inequality is also true 
% \begin{align}
% \|\gt(z) -\gt(z')\|^2 \geq  \alpha L ^2 \|z -z'\|^2,  \forall z, z' \in \mathbb R^{d},
% \end{align}
% then for arbitrarily close pairs of samples $(z-z)$ that $\|z-z'\| = o(\min(\|z\|,\|z'\|))$, where $ G(z')- G(z) \approx \nabla_z G(z)^T (z'-z)$, then we derive 
% \begin{align}\label{def:bound2}
% \|\nabla_z \gt(z)^T (z'-z)\|^2 \geq  \alpha L^2 \|z -z'\|^2.
% \end{align}
% This property could actually prevent the aforementioned degenerated case. For example, we construct $\tilde \gt(z')$ that $\tilde \gt(z')- \tilde \gt(z)=e_2^K$ where $e_2^K=[0,1,0,0,\cdots,0] \in \mathbb R^K$. We note such function cannot satisfy property in Eq.(\ref{def:bound2}). So we encourage the function to be sensitive to the variation along all the axis in the subspace of $\tilde \gt(z')$, however it should not be oversensitive to exceed a certain range. 

%\subsection{Safe Interpolation and Extrapolation}
%As we introduced before, we pursue valid interpolations to be valid within points in a local region, so we do not give more credit to those points $\gt(z)$ and $\gt(z')$ if they are distant from each other enough. 
Another side problem is how about to keep the semi-definiteness of the distance metric, to concord with metric learning research \cite{davis2007information, weinberger2006distance, weinberger2006unsupervised, xing2003distance}. Under this property, a pair of samples $(A,B)$ deviating from each other in whichever direction, should increase the pairwise distance in the output space. This property should also be enforced by diversification, although may not explicitly. This formulation of taking non-negative part of divergence loss encourages the learned metric space in $g(z)$ to be positive semidefinite (PSD). To understand our intuition with a counterexample, 
in a metric that% $d(z,z')=\Delta z^T W \Delta z, \where \Delta z=z-z'$
\begin{align}
    d(z,z')=\Delta z^T W \Delta z, \where \Delta z=z-z'
\end{align}
and the eigen-decomposition of $W$ is like %$ W=U^T diag[-\beta ,100\beta ,0,0,\cdots,0] U$, 
\begin{align}
    W=U^T diag[-\beta ,100\beta ,0,0,\cdots,0] U
\end{align}
where $\beta>0$ (eigen-decomposition), therefore $W$ is not PSD. Suppose there are two pairs $z_1,z_1',z_2,z_2'$ that $\Delta z_1=z_1-z_1'= U_1$ (the leading eigenvector) and $\tilde \Delta z_2= z_2-z_2'=U_2$ (the second eigenvector).  The two pairs incur a decrease of $99 \beta$ of $\ldiv$ in Eq.(\ref{eq::div}) without the nonnegative operator $\max(\cdot,0)$, which will give a unreasonable metric (non-positive-definite) if $\beta$ positively scales. However, if the operator is applied, the same case incurs an increase of $\beta$ of $\ldiv$ from the deviation in the subspace corresponds to the negative eigenvalue $-\beta$, as the $\max(\cdot,0)$ operator strongly contrast those subspace like $U_1$ that wrongly contribute to $\ldiv$, and ignore other subspace even if they correspond to strongly positive eigenvalues.

%However, these ideal properties may not be true in any region within the definition domain $\mathbb R^{d}$. This gives us an intuition to require the constraints to be satisfied in expectation,
%\begin{align}
%\mathbb E_{p } \max(\mathcal R(\theta, z,z'),0), \quad z,z'
%\end{align}
%w.r.t $p(z)$, the distribution of $z$ in which we are interested.% Since $z$ is generally sampled from a standard Gaussian distribution, we only need to consider the properties to hold in the concentrated area around the distribution of $z$, so we have access to judge whether the properties hold by sampling data points.

%\subsection{Application in GAN}
%For convenience, we denote the generator as $\gt$ and the discriminator as $\dt$, where $\theta$ and $\phi$  are the parameters of the two function respectively. The generator's functionality is to synthesize an image $y$ from a vector $z$, which is randomly sampled from a standard Gaussian distribution $\mathcal N(0, I)$, and $y$ should be as indistinguishable from the real images as possible. To distinguish generated images from real images obtained from cameras, the discriminator has to be fed with real images, and to be trained to make a binary classification about whether an image is realistic or not. The generator and discriminator are simultaneously trained in an adversarial fashion, so two models strengthen each other in the process.


%As the typical training process is based on alternating (stochastic) gradient descent, following this framework, in each step of updating $\phi$, we optimize it as usual; for updating $\theta$, we optimize the regularized form. 

%
%Our algorithm is summarized as follows,
%\begin{algorithm}
%	\caption{Training procedure for GAN}
%	\label{alg:the_alg}
%	\begin{algorithmic}[1]
%		%\Function{Iterative Pose Refine}{}
%		\While {not converged}
%		\State Sample a minibatch of data pairs:  $\{z_i, z_i'\}_{i=1}^M$,
%		\State Generate images with:  $\dt(y) = \dt(\gt(z))$ with $z$ sampled from $p$.
%		%		\State $\textbf{Given}: \textnormal{Reference-Target Pair: } (\mbox{I}_{ref}, \mbox{I}_{tar}), \textnormal{Default Pose Heatmap: } \mbox{P}_0$
%		\State Optimize w.r.t the discriminator $\phi =\phi +\eta \partial_{\phi} \mathcal L(\theta,\phi)$
%		\State Optimize w.r.t the discriminator $\theta =\theta -\eta
%		\partial_{\theta} \mathcal L(\theta,\phi) +\mathbb E_p[\max(\mathcal R(\theta, p),0)]$ 
%		\EndWhile
%		%\EndFunction
%	\end{algorithmic}
%\end{algorithm}  

%G: $z -> y$
%D: $y -> score$
%
%score $= D(y) = D(G(z))$
%
%In each epoch, we first sample ${z_i}$ to train the discriminator $D$ while fixing $G$
%
%2. Sample ${z_i}$, Fix $D$, Train $G$ w.r.t. Eq. followed
%
%$\min_{G }  \frac{2}{N(N-1)} \sum_{i,j}^N \textit{Relu}(\alpha\|z_i -z_j\|^2 - \|G(z_i) -G(z_j)\|^2)$
%
%3. Sample ${z_i}$, Fix D, Train G


%The divergence loss has the following form,
%\begin{align}
%\min_{G }  \frac{1}{N} \sum_{i,j}^N \textit{Relu}( \alpha\|z_i -z_j\|^2 - \|G(z_i) -G(z_j)\|^2) \nonumber \\ -D(x_i)log(D(x_i)) - (1- D(G(z_i)))log(1 - D(G(z_i)))
%\end{align}
